PhyMetric: Diagnosing Physical Plausibility in Text-to-Video Generation via Scene-Level QA

Text-to-video (T2V) generation models can produce visually realistic videos that nevertheless violate the physical consequences implied by the prompt and scene. Existing benchmarks largely rely on holistic plausibility scores or broad quality dimensions, leaving it unclear which physical behavior is being tested and why a model fails. We introduce PhyMetric, a scene-level diagnostic benchmark that recasts physical plausibility evaluation as verifiable, scene-grounded question answering. PhyMetric contains 1{,}115 scenes spanning 50 physical categories across six domains, paired with 8{,}920 answer-balanced binary questions over 12 evaluation dimensions. Each scene is associated with eight targeted yes/no questions and a structured physical prior specifying the governing law, expected temporal sequence, observable signatures, and common failure modes. At evaluation time, a vision-language model (VLM) judge answers each question from question-aware sampled frames conditioned on the prior, and correctness is hierarchically aggregated into scene, dimension, physical category, and model scores. Experiments on four open-source T2V models and three VLM judges show that scene-specific binary QA is a critical component of the protocol: when each targeted question is replaced by a single generic plausibility query, evaluator accuracy drops to the chance level. Structured physical priors offer a complementary signal that improves human alignment of the resulting scores, with effects that vary across VLM judges of different capacity. These findings establish PhyMetric as a benchmark that turns physical plausibility evaluation from opaque holistic scoring into interpretable, scene-level inspection. Our project page is available at: https://mengsiwei.github.io/PhyMetric/.

==> sections/03phymetricBenchmark.tex <==
\section{\phymetric{} Benchmark Construction}
\label{sec:construction}

\subsection{Overview}
A reliable physical benchmark ideally satisfy three competing goals, namely broad domain coverage, namely broad domain coverage, scene-specific physical consequences rather than coarse realism, and a balanced and reproducible curation pipeline.
\phymetric{} addresses these requirements through a three-stage construction pipeline that proceeds from a structured physics taxonomy, through LLM-based scene and question synthesis, to expert verification (Figure~\ref{fig:}).


As shown in Figure~\ref{fig:taxonomy}, we define \textbf{50 physical categories} spanning \textbf{6 major physics domains}: mechanics, fluid dynamics, materials, thermal processes, electromagnetism, and chemistry.
Each category is associated with an explicit physical principle, an object pool, an environment pool, and key diagnostic dimensions.
We then expand each category into \textbf{20--30 diverse scenes} with different objects, settings, and visual contexts.
For each scene, we construct a detailed generation prompt and a causal chain describing the initial state, physical process, and expected final state.
This design provides broad scene diversity while keeping the underlying physical event well defined.

For question construction, we first use a GPT-based LLM~\cite{} to generate coarse scene-specific binary questions from the category metadata.
Each scene is paired with \textbf{8 yes/no questions}, including both positive questions that describe expected physical outcomes and negative questions that describe plausible failure modes.
The yes/no labels are balanced within each scene to reduce answer-prior bias.
Questions are also assigned difficulty levels from easy, medium, and hard, and they cover multiple physical dimensions such as motion, direction, interaction, causality, shape, material, spatial relation, number, and appearance.
After automatic generation, three physics experts manually review the coarse questions.
They filter out ambiguous, visually unverifiable, redundant, or physically incorrect questions, and revise questions whose wording may leak the answer or depend on information not visible in the generated video.
The experts also check whether the assigned labels are correct, whether positive and negative questions are balanced, and whether the selected frame indices are appropriate for the targeted physical event.
Only questions that pass this expert verification are kept in the final benchmark.

Following this process, \phymetric{} contains \textbf{50 physical categories}, \textbf{1,115 benchmark scenes}, and \textbf{8,920 expert-verified binary questions} in total, with each scene paired with 8 balanced diagnostic questions.
This final curation preserves broad physical diversity while maintaining question quality, label balance, and diagnostic reliability.
PhyMetric transforms physical video benchmarking from small-scale, narrow, or subjective evaluation into a structured and scalable benchmark with:
(i) broad domain coverage,
(ii) scene-level causal grounding,
(iii) balanced binary QA,
and (iv) dimension-level diagnostic diversity.
This construction enables PhyMetric to serve not only as an evaluation benchmark, but also as a diagnostic framework for systematically probing which physical capabilities remain challenging for modern text-to-video models.


\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/fig_construction.pdf}
    \caption{\small\textbf{\phymetric{} taxonomy and benchmark construction.}
    \phymetric{} covers 50 physical categories across six physics domains.
    Each category is expanded into diverse scenes with causal chains, generation prompts, and balanced scene-specific binary questions.}
    \label{fig:taxonomy}
\end{figure}

% \paragraph{Physics Taxonomy.}
% We first organize physical phenomena into a taxonomy covering six domains:
% \textit{mechanics}, \textit{fluids}, \textit{materials}, \textit{thermal processes}, \textit{electromagnetism}, and \textit{chemistry}.
% As shown in Figure~\ref{}, these domains are further divided into 50 physical categories.
% The category set is designed to cover the types of dynamics that are commonly exposed in generated videos, including motion under force, fluid behavior, material deformation, state transition, and chemical change.
% This taxonomy is therefore not used as a topic list, but as a coverage map that ensures \phymetric{} evaluates diverse forms of physical behavior rather than overfitting to a few familiar motions such as falling or bouncing.

% \paragraph{Scene Construction.}
% For each category, we create scene instances by specifying the objects, environment, initial condition, physical process, and expected outcome.
% The bottom part of Figure~\ref{} shows the event-level view.
% Each scene is associated with a short temporal script that describes what should be visible at early, middle, and late stages of the video.
% For example, a buoyancy scene should show placement in fluid, floating or sinking behavior, and a stable final relation between the object and the liquid surface.
% The temporal script provides the bridge between abstract physical laws and visual evidence.

% \paragraph{Binary Question Design.}
% We then derive binary yes/no questions from each scene-level temporal script.
% Each question targets one observable consequence of the expected process, such as motion direction, contact, deformation, material response, object persistence, state change, or causal order.
% The questions are scene-specific rather than generic physics quizzes.
% For instance, the benchmark asks whether a particular object accelerates downward after release, whether two objects rebound after contact, or whether a material visibly deforms after impact.
% This design makes the score diagnostic: an incorrect answer can be linked to a concrete physical consequence instead of only indicating that the whole video ``looks implausible''.
% Across the benchmark, yes and no labels are balanced to keep the chance baseline interpretable and to reduce answer-prior bias.

% \paragraph{Structured Prompting Package.}
% Finally, each scene is paired with a physics-grounded structured prompting package.
% This package is a scene-level knowledge base generated from text only.
% It specifies the governing physical principle, the expected temporal sequence, key physical signatures, common failure modes, and dimension-specific hints for judging.
% During evaluation, this knowledge base anchors the VLM judge to the physical expectation implied by the scene before it answers the binary questions.
% In this way, \phymetric{} turns physical plausibility evaluation into grounded verification over explicit scene-level consequences, rather than a post hoc holistic impression of the generated clip.

% Unlike existing benchmarks that rate each video with a holistic Likert score~\cite{} or a single global rule~\cite{}, \phymetric{} decomposes physical plausibility into binary scenario-specific questions tied to concrete physical laws, which enables fine-gained diagnosis of what kind of physics a generator fails on.


% \subsection{Physics Taxonomy}
% \label{subsec:physicsTaxonomy}



% \subsection{Scene and Question Design}
% \label{subsec:questions}

% \paragraph{Scene construction.}


% \paragraph{Question design.}



% \subsection{Knowledge Base Construction}
% \label{subsec:kbConstruction}



% \begin{table}[t]
% \centering
% \caption{PhyMetric benchmark statistics.}
% \label{tab:phymetric_stats}
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{lr}
% \toprule
% Physical phenomena (categories)   & 50 \\
% Scenes                             & 1{,}115 \\
% Questions                          & 8{,}920 \\
% Questions per scene                & 8  (4 yes + 4 no)\\
% Physical dimensions                & 12 \\
% Difficulty levels                  & 3  (easy / medium / hard) \\
% Video specification                & 30 fps, 4\,s, 120 frames \\
% Answer balance                     & 50\% yes / 50\% no \\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[t]
% \centering
% \caption{Comparison with existing physical video benchmarks.}
% \label{tab:benchmark_compare}
% \setlength{\tabcolsep}{4pt}
% \footnotesize
% \begin{tabular}{lccccc}
% \toprule
% Benchmark & Scenes & Questions & Format & Law-grounded & Balanced \\
% \midrule
% PhyGenBench~\cite{}      & 160   & --    & 1 rule / video & \checkmark & -- \\
% VideoPhy~\cite{}            & 688   & --    & Likert 1–5     & --         & -- \\
% VideoPhy-2~\cite{}         & 3{,}940 & --  & Likert 1–5 + rules & partial & -- \\
% ETVA~\cite{}                    & 2{,}000 & 12K & Yes/No         & --          & --  \\
% \textbf{PhyMetric} (ours)           & \textbf{1{,}115} & \textbf{8{,}920} & Yes/No & \checkmark & \checkmark \\
% \bottomrule
% \end{tabular}
% \end{table}

==> sections/04evaluation.tex <==
\section{Evaluation Methodology}
\label{sec:eval}

Evaluating physical plausibility in text-to-video generation is fundamentally different from measuring visual realism alone.
As shown in Figure~\ref{fig:teaser_overview}, a generated video may appear globally plausible under holistic judgment while still violating critical scene-specific physical consequences. 
This mismatch shows that existing holistic evaluation paradigms does not necessarily imply physical correctness. 
Generic questions tend to encourage confidence-driven judgments and overlook localized physical failures, leading to unstable or misleading assessments.
\phymetric{} addresses this issue by replacing holistic plausibility scoring with scene-level diagnostic QA.
Instead of asking whether a whole video is physically plausible, we ask a set of scene-specific binary questions, each targeting a verifiable physical consequence.
These questions cover observable properties from 12 physical motion dimensions, such as motion quality, object persistence, and state transition.
As illustrated in Figure~\ref{fig:evaluation_pipeline}, the evaluation consists of three steps: (1) scene definition and video evidence extraction, (2) scene-specific physical context, and (3) VLM answering with score aggregation.

% Given a generated video $V_s$ for scene $s$, \phymetric{} evaluates physical plausibility through scene-specific binary questions.
% Each question targets an observable physical consequence implied by the scene, such as motion direction, contact, deformation, material response, object persistence, state transition, or causal order. 
% The final score aggregates correctness over these targeted checks. 
% This design makes the tested physical consequence identifiable, and it grounds the evaluator in the physical expectation of the scene before video-based answering.

% \subsection{Frame Sampling}
% \label{subsec:frameSampling}
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/fig_evaluation.pdf}
    \caption{\small\textbf{\phymetric{} evaluation pipeline.}
    For each physical scene $s$, a text-to-video generates a video $V_s$ from the scene caption $c_s$.
    Given $V_s$, question-aware frames are sampled to each scene-specific binary question $q_i^{(s)}$ for next step setup.
    A structured physical prior $K_s$ is then constructed from the scene description to summarize the expected physical law, target outcome, and common failure modes.
    In the final step, a vision-language model (VLM) answers all questions conditioned on both sampled frames and $K_s$.
    Each question is scored against ground-truth labels to produce question-level correctness, which is averaged into a scene score  $S(s, V_s)$.
    % $S(s, V_s)=\frac{1}{N_s}\sum_{i=1}^{N_s}\mathbb{I}[\hat{a}_i^{(s)}=a_i^{(s)}]$. 
    The model performance is computed by averaging scene scores across all benchmark scenes.
    This hierarchical design transforms holistic video evaluation into scene-grounded physical diagnosis through structured priors, question-specific evidence, and interpretable multi-level scoring.
    }
    \label{fig:evaluation_pipeline}
\end{figure}


\paragraph{Scene-Level QA Formulation.}

Each scene $s$ contains a scene caption $c_s$, a generated video $V_s$, a set of binary questions
$\mathcal{Q}_s=\{q_i^{(s)}\}_{i=1}^{N_s}$, question-specific reference frame indices, and ground-truth answers $\{a_i^{(s)}\}_{i=1}^{N_s}$.
Across the benchmark, yes/no labels are balanced to keep chance performance interpretable and reduce answer-prior bias.
For each question $q_i^{(s)}$, the evaluator predicts a binary answer $\hat{a}_i^{(s)} \in \{0,1\}$ using sampled visual evidence and scene-specific physical context.
We score each answer by exact match with the ground-truth label and compute the scene score as
\[
S(s,V_s)=\frac{1}{N_s}\sum_{i=1}^{N_s}
\mathbb{I}\!\left[\hat{a}_i^{(s)}=a_i^{(s)}\right],
\]
where $\hat{a}_i^{(s)}$ is the predicted answer and $a_i^{(s)}$ is the ground-truth label.
The final model score is obtained by averaging $S(s,V_s)$ over all scenes.

% think here : this paragraph should be moved to section 3
\paragraph{Structured Physical Prior Construction.}

To ground the evaluator before video inspection, each scene is paired with a structured physical prior $K_s$.
This prior is generated from the scene caption $c_s$ only and is independent of the generated video $V_s$.
It summarizes the relevant physical law or principle, the expected outcome, observable evidence, and common failure modes.
For example, in the tomato-slicing scene, $K_s$ may encode that the knife should cut through the tomato, the whole tomato should separate into two parts, and common failures include floating pieces, wrong object count, or missing interior texture.
The purpose of $K_s$ is not to provide the answer directly, instead, it specifies what physical behavior should be checked.
This separates expectation construction from visual verification and reduces the risk that the VLM judge is biased by visual artifacts or generic plausibility priors.


\paragraph{Question-Aware Frame Sampling.}
For each question $q_i^{(s)}$, \phymetric{} samples frames from the generated video according to question-specific reference frame indices.
This differs from uniform video sampling, since different questions may require evidence from different moments.
For example, a question about initial contact may focus on early frames, while a question about final separation may require late frames.
Since generated videos may have different lengths and frame rates, we map a reference frame index $f$ from a reference clip with $N_{\mathrm{ref}}$ frames to a generated video with $N_V$ frames as
\[
f' =
\mathrm{round}
\left(
\frac{f}{N_{\mathrm{ref}}-1}(N_V-1)
\right).
\]
For each mapped index $f'$, we extract the target frame and its neighboring frames when available.
This gives the evaluator local temporal evidence around the queried physical event instead of a single isolated image.


\paragraph{Frame-Grounded VLM Answering and Score Aggregation.}
\label{subsec:answering}
In the final step of \phymetric{}, the VLM evaluator receives four inputs:
the sampled frames $\mathcal{F}_i^{(s)}$, the scene caption $c_s$, the structured prior $K_s$, and the binary question $q_i^{(s)}$.
It is instructed to output a yes/no answer, a confidence score, and a short explanation. 
The answer is parsed into $\hat{a}_i^{(s)}$ and compared against the ground-truth label $a_i^{(s)}$.
We report overall accuracy across all questions as the primary metric.
To support fine-grained analysis, we also compute scores by physical category, evaluation dimension, and difficulty level.
These diagnostic scores allow us to identify whether a model fails on specific dimension.
This allows \phymetric{} to distinguish not only which model performs better overall, but also which physical abilities remain difficult for current text-to-video models.

==> sections/05experiments.tex <==
\section{Experiments}
\label{sec:exp}

We evaluate \phymetric{} from three perspectives. 
First, we test whether the benchmark can distinguish current open-source text-to-video models on the full 1,115-scene benchmark. 
Second, we study which physical dimensions and domains remain most challenging. 
Third, we validate the benchmark design through human study and ablation experiments on a controlled 100-scene subset sampled as two scenes per category from all 50 categories, which preserves category-level coverage while keeping manual annotation and multi-condition ablation feasible.

\subsection{Experimental Setup}
\label{subsec:experimentalSetup}


We evaluate four open-source text-to-video models, CogVideoX-5B~\cite{yang2024cogvideox_iclr2025}, Wan2.1-1.3B~\cite{wan2025wan_arxiv2025}, Wan2.2-14B~\cite{wan2025wan_arxiv2025}, and Cosmos-7B~\cite{agarwal2025cosmos_arxiv2025}. 
Each model generates one video per scene using the scene caption as the input prompt, without model-specific prompt rewriting.
The full \phymetric{} benchmark contains 1,115 scenes from 50 physical categories and is used for the main model evaluation.

For evaluation, each question provides reference frame indices indicating when the relevant physical evidence should be inspected.
We map these indices proportionally to each generated video and sample local neighboring frames around the mapped positions.
The VLM judge receives these frames, the scene caption, the binary question, and the physics-grounded structured prompt.
We use Qwen3.5-9B~\cite{yang2025qwen3} as the default judge and include Qwen2.5-VL-7B-Instruct~\cite{bai2025qwen2}, and GPT-5.4~\cite{singh2025openai_gpt5} for cross evaluator and ablation analysis.
The physics-grounded structured prompts are generated by auxiliary text LLMs.
Each structured prompt contains the governing law, expected temporal sequence, and common failure modes for the corresponding scene.
To avoid a circular evaluation protocol, the structured prompt generator is separated from the VLM judge whenever possible, and we additionally test multiple prompt sources, including Qwen3.5~\cite{yang2025qwen3}, Qwen2.5~\cite{bai2025qwen2}, DeepSeek~\cite{guo2025deepseek_r1}, and Mistral~\cite{jiang20236g_mistral7B}.
This allows us to measure whether the evaluation depends on a particular knowledge-base generator or on the judge's own prior knowledge.
For human validation and ablation studies, we sample a controlled 100-scene subset with two scenes from each category.
In human study, 50 annotators watch the generated videos in the 100-scene subset and answer the same yes/no questions.

% \paragraph{VLM judges.}
% We evaluate generated videos using three VLM judges. Each judge receives sampled video frames, the scene caption, the binary question, and, in the full protocol, the physics-grounded structured prompt. The judge outputs a yes/no answer, confidence, and a short reason. We report accuracy against the ground-truth labels.

% \paragraph{Human study.}
% Human annotation is conducted on the 100-scene subset. The goal is not to compare humans and video models directly. Instead, human results are used to verify the validity of the QA protocol, estimate question difficulty, and assess whether the benchmark questions are answerable and meaningful to human observers.


\subsection{\phymetric{} Main Results}
\label{subsec:phymetricResults}

\paragraph{Full benchmark.}
% Table~\ref{tab:main_results} reports the overall scores of four text-to-video models on the full 1,115-scene benchmark. 
% The results show that \phymetric{} can separate current open-source models while remaining far from saturated. 
% Higher-scoring models tend to preserve event progression and material behavior more consistently, but all models still show visible failure modes in specific domains. 
% The ranking also suggests that physical plausibility does not follow parameter count alone. 
% Model family, training data, temporal modeling, and instruction-following behavior may all affect performance.

Table~\ref{tab:main_results} shows that \phymetric{} separates current open-source T2V models with a 7.25-point gap between the strongest and weakest systems.
Wan2.2-14B~\cite{wan2025wan_arxiv2025} obtains the highest overall score, followed by Cosmos-7B~\cite{agarwal2025cosmos_arxiv2025}, Wan2.1-1.3B~\cite{wan2025wan_arxiv2025}, and CogVideoX-5B~\cite{yang2024cogvideox_iclr2025}.
As shown in Figure~\ref{fig:dim_radar}, higher-scoring models tend to preserve more accurate material behavior and motion consistency.

The ranking is not explained by parameter count alone: CogVideoX-5B is larger than Wan2.1-1.3B, yet scores lower.
This suggests that \phymetric{} captures differences in temporal modeling, training data, and physical event synthesis rather than only model scale.

\paragraph{Controlled 100-scene subset.}


% \begin{table}[t]
% \centering
% \caption{
% \small
% Main results on the full \phymetric{} benchmark under the full evaluation protocol.
% We report overall accuracy, combined weighted accuracy, and accuracy by question difficulty.
% }
% \label{tab:main_results}
% \setlength{\tabcolsep}{5pt}
% \resizebox{0.55\columnwidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
% Model & Overall & Weighted & Easy & Medium & Hard \\
% \midrule
% Wan2.2-14B    & \textbf{77.88} & \textbf{79.23} & \textbf{76.15} & \textbf{72.88} & 85.71 \\
% Cosmos-7B     & 76.50 & 77.54 & 75.00 & \textbf{72.88} & 82.45 \\
% Wan2.1-1.3B   & 74.62 & 76.85 & 66.54 & 72.20 & \textbf{86.12} \\
% CogVideoX-5B  & 70.63 & 72.45 & 66.54 & 66.78 & 79.59 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

\begin{table}[t]
\centering
\caption{
Main results on the full \phymetric{} benchmark (1{,}115 scenes) using open-source VLM evaluators. 
\emph{Average} denotes the mean performance across Qwen3.5 and Qwen2.5-VL.
}
\label{tab:results_full}
\small
\setlength{\tabcolsep}{4pt}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Qwen3.5-9B}} & \multicolumn{2}{c}{\textbf{Qwen2.5-VL-7B}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& Overall & Weighted & Overall & Weighted & Overall & Weighted \\
\midrule
Wan2.2-14B   & \textbf{76.74} & \textbf{78.07} & 68.82          & 70.82          & \textbf{72.78} & \textbf{74.45} \\
Cosmos-7B    & 76.28          & 77.60          & \textbf{68.89} & \textbf{70.92} & 72.59          & 74.26          \\
Wan2.1-1.3B  & 73.86          & 75.50          & 67.26          & 69.42          & 70.56          & 72.46          \\
CogVideoX-5B & 71.36          & 73.18          & 65.12          & 67.62          & 68.24          & 70.40          \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[t]
\centering
\caption{
Evaluation on the 100-scene controlled subset across both closed and open-source VLM evaluators. 
\emph{Average} reflects the mean accuracy across all three judges.
}
\label{tab:results_subset}
\small
\setlength{\tabcolsep}{3pt}
\resizebox{0.84\columnwidth}{!}{%
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Qwen3.5-9B}} & \multicolumn{2}{c}{\textbf{Qwen2.5-VL-7B}} & \multicolumn{2}{c}{\textbf{GPT-5.4}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& Overall & Weighted & Overall & Weighted & Overall & Weighted & Overall & Weighted \\
\midrule
Wan2.2-14B   & \textbf{77.88} & \textbf{79.23} & 66.75          & 69.54          & 73.12          & 74.26          & 72.58          & 74.34          \\
Cosmos-7B    & 76.50          & 77.54          & \textbf{67.37} & \textbf{70.37} & \textbf{74.00} & \textbf{75.54} & \textbf{72.62} & \textbf{74.48} \\
Wan2.1-1.3B  & 74.62          & 76.85          & 65.87          & 68.94          & 72.12          & 73.88          & 70.87          & 73.22          \\
CogVideoX-5B & 70.63          & 72.45          & 64.38          & 67.13          & 69.75          & 71.67          & 68.25          & 70.42          \\
\bottomrule
\end{tabular}%
}
\end{table}

% \begin{table}[t]
% \centering
% \caption{
% Main results on \phymetric{} under the full evaluation protocol.
% \emph{Top block:} full benchmark (1{,}115 scenes from 50 categories).
% \emph{Bottom block:} controlled 100-scene subset (two scenes per category) used for human study and ablation.
% For each video model and each VLM judge we report \emph{Overall} and \emph{Weighted} accuracy (\%).
% The Qwen3.5-9B columns reflect the default judge used elsewhere in the paper; the Qwen2.5-VL and GPT-5.4 columns assess robustness to evaluator choice.
% The \emph{Average} columns are the unweighted mean across the three VLM judges.
% }
% \label{tab:main_results}
% \small
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.05}
% \begin{tabular}{lcc cc cc cc}
% \toprule
% \multirow{2}{*}{\textbf{Model}}
%   & \multicolumn{2}{c}{\textbf{Qwen3.5-9B}}
%   & \multicolumn{2}{c}{\textbf{Qwen2.5-VL-7B}}
%   & \multicolumn{2}{c}{\textbf{GPT-5.4}}
%   & \multicolumn{2}{c}{\textbf{Average}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
%  & Overall & Weighted & Overall & Weighted & Overall & Weighted & Overall & Weighted \\
% \midrule
% \multicolumn{9}{l}{\textit{Full benchmark (1{,}115 scenes / 8{,}920 questions)}} \\
% Wan2.2-14B   & \textbf{76.74} & \textbf{78.07} & 68.82 & 70.82 & -- & -- & -- & -- \\
% Cosmos-7B    & 76.28 & 77.60 & \textbf{68.89} & \textbf{70.92} & -- & -- & -- & -- \\
% Wan2.1-1.3B  & 73.86 & 75.50 & 67.26 & 69.42 & -- & -- & -- & -- \\
% CogVideoX-5B & 71.36 & 73.18 & 65.12 & 67.62 & -- & -- & -- & -- \\
% \cmidrule(lr){1-9}
% \textit{Mean (4 models)} & 74.56 & 76.09 & 67.52 & 69.70 & -- & -- & -- & -- \\
% \midrule
% \multicolumn{9}{l}{\textit{100-scene subset (two scenes per category / 800 questions)}} \\
% Wan2.2-14B   & \textbf{77.88} & \textbf{79.23} & 66.75 & 69.54 & 73.12 & 74.26 & 72.58 & 74.34 \\
% Cosmos-7B    & 76.50 & 77.54 & \textbf{67.37} & \textbf{70.37} & \textbf{74.00} & \textbf{75.54} & \textbf{72.62} & \textbf{74.48} \\
% Wan2.1-1.3B  & 74.62 & 76.85 & 65.87 & 68.94 & 72.12 & 73.88 & 70.87 & 73.22 \\
% CogVideoX-5B & 70.63 & 72.45 & 64.38 & 67.13 & 69.75 & 71.67 & 68.25 & 70.42 \\
% \cmidrule(lr){1-9}
% \textit{Mean (4 models)} & 74.91 & 76.52 & 66.09 & 69.00 & 72.25 & 73.84 & 71.08 & 73.12 \\
% \bottomrule
% \end{tabular}
% \end{table}

\subsection{Dimension-Level Analysis}
\label{subsec:dimensionAnalysis}

Table~\ref{tab:dimension_analysis} breaks down performance across 12 evaluation dimensions.
The strongest dimensions are \textit{number} and \textit{direction}, while the lowest dimensions are perception-related \textit{appearance} and \textit{size}.
The average accuracy on \textit{number} reaches 90.39\%, suggesting that current T2V models and VLM judges can often verify object count when the relevant evidence is visually clear.
Direction and motion also score above 79\%, which indicates that coarse kinematic patterns are relatively well captured.
The weakest performance on \textit{appearance} suggests that physical failures often appear as material or state inconsistency rather than only wrong motion. 
% For example, a melting object may change shape without a correct liquid state, a deformable object may lose texture identity, or a fluid may appear visually present but fail to show the expected mixing or surface behavior.
\textit{Size} and \textit{spatial} reasoning are also weak, which reflects persistent problems in preserving object scale and object relative placement over time.
The inter-model spread further reveals which dimensions best distinguish generators.
Appearance/texture and shape have spreads of 10.00 and 10.53 points, respectively, while object identity has only a 1.69-point spread.
This means that the four models are similar on some basic object-level checks, but differ more strongly on material appearance and deformation-related physical behavior.


Figure~\ref{fig:dim_radar} further visualizes the dimension profiles of the four evaluated T2V models.
Wan2.2-14B forms the broadest and most stable profile, with strong coverage on kinematic and causal dimensions.
Cosmos-7B attains the largest number of dimension-wise best scores, indicating that it is highly competitive on specific physical checks even through its overall score is slightly below Wan2.2-14B.
Wan2.1-1.3B shows a more selective profile on material and existence dimensions,
while CogVideoX-5B shows a visibly contracted profile, especially in dimensions that require stable physical appearance or relational evidence.
This visualization suggests that model differences are not only scalar, but also structural, in which two models with close overall scores may succeed on different types of physical evidence.


\begin{figure*}[t]
    \centering
    \begin{minipage}[c]{0.33\textwidth}
        \centering
        \small
        \captionof{table}{Dimension-level performance averaged over four T2V models.}
        \label{tab:dimension_analysis}
        \setlength{\tabcolsep}{4pt}
        \renewcommand{\arraystretch}{1.0}
        \begin{tabular}{lcc} 
            \toprule
            \textbf{Dimension} & \textbf{Avg. Acc.} & \textbf{Spread} \\
            \midrule
            Number & \textbf{90.39} & 3.85 \\
            Direction & 81.41 & 7.70 \\
            Motion & 79.59 & 8.21 \\
            Material & 77.22 & 8.89 \\
            Shape & 76.97 & \textbf{10.53} \\
            Causal & 76.72 & 7.64 \\
            Existence & 75.19 & 9.78 \\
            Object & 75.00 & 1.69 \\
            Interaction & 73.24 & 5.53 \\
            Spatial & 72.17 & 5.21 \\
            Size & 69.74 & 7.89 \\
            Appearance & \textbf{66.39} & 10.00 \\
            \bottomrule
        \end{tabular}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.63\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/fig_dim_radar.pdf}
        \caption{\small \textbf{Dimension-level capability profiles of four T2V models on \phymetric{}.} 
        The left radar plot compares all models across the 12 evaluation dimensions, and the right four smaller plots show each model separately.
        % Filled markers on right figures indicate dimensions where a model obtains the best score among the four models.
        The visualization emphasizes the structure of each model's physical profile.
        }
        \label{fig:dim_radar}
    \end{minipage}
\end{figure*}

\subsection{Ablation Study}
\label{subsec:ablation}

We conduct ablations on the 100-scene subset to examine the two main design choices of \phymetric{}: scene-specific QA and the structured physical prior.
For each scene $s$, the structured physical prior $K_s$ is generated before video evaluation from the scene description and category metadata.
% It specifies the governing physical law, expected temporal sequence, observable physical signatures, common failure modes, and dimension-specific hints.
Importantly, $K_s$ is generated without access to the generated videos or ground-truth question answers, which provides scene-level expectation grounding for VLM judge.

\paragraph{Component ablation.}

Table~\ref{tab:ablation_components} studies the interaction between question specificity and $K_s$.
The most consistent finding is that scene-specific QA is the load-bearing component of \phymetric{}.
When the original questions are replaced by a single generic query, \textit{``Is this video physically plausible?''}, the accuracy drops close to the 50\% chance level across all evaluators, which means the evaluators are retrogress to chance-level behavior.
Without scene-specific questions, both evaluator cannot reliably map the video evidence to the intended physical consequence, and its yes/no decisions become no more informative than random guessing.
For example, without $K_s$, Qwen3.5-9B drops from 72.75\% with scene-specific QA to 48.13\% with generic QA, Qwen2.5-VL drops from 63.47\% to 47.31\%, and GPT-5.4 drops from 73.94\% to 49.25\%.
Adding $K_s$ to the generic question does not recover the missing signal.
This shows that a holistic plausibility query cannot identify which physical consequence is being tested, even when extra physical context is available.
The human-correlation also proves the validity of our scene-specific question design.
For Qwen3.5-9B, the full setting improves both accuracy and human alignment over the no-$K_s$ scene-specific setting, increasing \(\rho_{\text{human}}\) from 0.165 to 0.201.
For GPT-5.4, adding $K_s$ slightly reduces benchmark-label accuracy, but improves human alignment from 0.216 to 0.250 and reaches statistical significance.
% For Qwen2.5-VL, the highest human correlation appears in the no-$K_s$ scene-specific setting, although $K_s$ still improves accuracy.
These patterns show that accuracy and human alignment capture related but distinct aspects of evaluator behavior.
Most importantly, the scene-specific setting consistently provides high diagnostic accuracy, while the structured prior can improve human alignment for stronger evaluators.

\textcolor{red}{
The structured physical prior has a smaller and evaluator-dependent effect when the scene-specific questions are kept.
% With scene-specific questions fixed, adding $K_s$ improves label accuracy for Qwen3.5-9B from 72.75\% to 74.91\%, and for Qwen2.5-VL from 63.47\% to 66.09\%.
% For GPT-5.4, however, accuracy decreases from 73.94\% to 72.25\%.
% To verify the effectiveness of
% Human correlation reveals a second pattern.
% For GPT-5.4, adding $K_s$ improves $\rho_{\text{human}}$ from 0.216 to 0.250, even though accuracy decreases.
% For Qwen3.5-9B and Qwen2.5-VL, the highest human correlation appears in the no-$K_s$ scene-specific condition.
% These results suggest that $K_s$ is not a universal accuracy booster.
% Rather, it provides expectation grounding that can help or hurt depending on the evaluator's ability to reconcile textual physical priors with visual evidence.
% Overall, Table~\ref{tab:ablation_components} supports the central design of \phymetric{}.
% Scene-specific QA addresses the identifiability problem by specifying the physical consequence under test.
% The structured physical prior addresses expectation grounding, but its benefit depends on the evaluator.
% The collapse of generic QA with and without $K_s$ shows that expectation grounding cannot replace identifiable, scene-level questions.
}



\begin{table}[t]
  \centering
  \caption{\small\textbf{Component ablation of \textsc{PhyMetric}.}
  We toggle the structured physical prior $K_s$ and the question style.
  ``Scene-specific'' denotes our targeted binary questions, while ``Generic''
  replaces each question with a single global plausibility query.
  \emph{Overall} and \emph{Weighted} are mean accuracies (\%) across four
  T2V generators. 
  $\rho_{\text{human}}$ is the scene-level Spearman correlation with the
  human study, averaged over four video generators.
  The results show that scene-specific questions are necessary for diagnostic
  accuracy, while $K_s$ has evaluator-dependent effects on accuracy and
  human alignment.}
  \label{tab:ablation_components}
  \small
  \setlength{\tabcolsep}{12pt}
  \renewcommand{\arraystretch}{1.05}
  \begin{tabular}{ccl ccc} % 列格式已修改为 ccc
    \toprule
    \textbf{$K_s$} & \textbf{Question} & \textbf{Evaluator}
    & \textbf{Overall} & \textbf{Weighted}
    & \textbf{$\rho_{\text{human}}$} \\ % 已删去 \Delta
    \midrule
    \ding{51} & Scene-specific & Qwen3.5-9B & \textbf{74.91} & \textbf{76.52} & \textbf{+0.201} \\
    \ding{55} & Scene-specific & Qwen3.5-9B & 72.75 & 74.56 & +0.165 \\
    \ding{55} & Generic        & Qwen3.5-9B & 48.13 & 49.71 & +0.192 \\
    \ding{51} & Generic        & Qwen3.5-9B & 48.88 & 50.17 & +0.196 \\
    \midrule
    \ding{51} & Scene-specific & Qwen2.5-VL & \textbf{66.09} & \textbf{69.00} & +0.104 \\
    \ding{55} & Scene-specific & Qwen2.5-VL & 63.47 & 65.89 & \textbf{+0.215} \\
    \ding{55} & Generic        & Qwen2.5-VL & 47.31 & 50.36 & +0.139 \\
    \ding{51} & Generic        & Qwen2.5-VL & 46.91 & 50.64 & +0.030 \\
    \midrule
    \ding{51} & Scene-specific & GPT-5.4 & 72.25 & 73.84 & \textbf{+0.250}$^{*}$ \\
    \ding{55} & Scene-specific & GPT-5.4 & \textbf{73.94} & \textbf{75.28} & +0.216 \\
    \ding{55} & Generic        & GPT-5.4 & 49.25 & 49.30 & +0.121 \\
    \ding{51} & Generic        & GPT-5.4 & 47.12 & 48.45 & +0.202 \\
    \bottomrule
  \end{tabular}
  \vspace{2pt}
  \begin{flushleft}
  \footnotesize{$^{*}$ marks $p<0.05$.}
  \end{flushleft}
\end{table}

\paragraph{Effect of structured physical prior source and evaluator.}
To test whether the structured physical prior depends on a particular LLM source, we generate $K_s$ with different auxiliary LLMs and evaluate them with different VLM judges in Table~\ref{tab:ablation_kb_eval}.
For Qwen3.5-9B as evaluator, all structured priors improve both accuracy and human correlation over zero-shot.
The DeepSeek and Mistral priors yield the strongest human correlations on Qwen3.5-9B evaluator with 0.251 and 0.248 compared to Qwen-series priors, which indicate that cross-source priors improve the alignment with human judgments.
The trend also reflects on Qwen2.5-VL evaluator, where the DeepSeek prior gives the highest human correlation.
For GPT-5.4, zero-shot gives the highest accuracy, but every structured prior improves human correlation, with the Mistral prior reaching the best \(\rho_{\text{human}}=0.293\).
This is important for the goal of \phymetric{} that a useful metric should not only match benchmark labels, but also track human-perceived physical plausibility.
The results suggest that structured physical priors can make evaluator judgments more human-aligned, especially for stronger evaluators, even when they do not maximize raw accuracy.
Overall, these ablations show that \phymetric{} is valid as a diagnostic metric because its core scene-specific QA remains necessary for accuracy, and its structured physical prior provides an additional path toward human-aligned physical judgment.

\begin{table}[t]
  \centering
  \caption{\small\textbf{Effect of structured physical prior source and evaluator.}
  Each row is a pair of prior source and question evaluator.
  \emph{zero-shot} means without the structured physical prior $K_s$.
  \emph{Overall} and \emph{Weighted} are mean accuracies (\%) across four
  T2V generators. $\rho_{\text{human}}$ is the scene-level Spearman correlation
  with the human study.
  Cross-source priors improve Qwen3.5-9B accuracy and improve GPT-5.4
  human correlation, suggesting that the effect of $K_s$ is not merely due
  to self-evaluation, but depends on evaluator capacity and prompt
  compatibility.}
  \label{tab:ablation_kb_eval}
  \small
  \setlength{\tabcolsep}{8pt}
  \renewcommand{\arraystretch}{1.05}
  \begin{tabular}{ll ccc} % 这里的列格式由 cccc 改为 ccc
    \toprule
    \textbf{$K_s$ source} & \textbf{Evaluator}
    & \textbf{Overall} & \textbf{Weighted}
    & \textbf{$\rho_{\text{human}}$} \\ % 已删去 \Delta
    \midrule
    \textit{zero-shot} & Qwen3.5-9B & 72.75 & 74.56 & +0.165 \\
    Qwen3.5-9B & Qwen3.5-9B & \textbf{74.91} & \textbf{76.52} & +0.201 \\
    Qwen2.5-7B-Instruct & Qwen3.5-9B & 73.66 & 75.42 & +0.209 \\
    DeepSeek-R1-Distill-Llama-8B & Qwen3.5-9B & 73.81 & 75.67 & \textbf{+0.251}$^{*}$ \\
    Mistral-7B-Instruct-v0.3 & Qwen3.5-9B & 74.09 & 76.13 & +0.248$^{*}$ \\
    \midrule
    \textit{zero-shot} & Qwen2.5-VL & 63.47 & 65.89 & +0.015 \\
    Qwen3.5-9B & Qwen2.5-VL & \textbf{66.09} & \textbf{69.00} & +0.104 \\
    Qwen2.5-7B-Instruct & Qwen2.5-VL & 63.25 & 66.15 & +0.156 \\
    DeepSeek-R1-Distill-Llama-8B & Qwen2.5-VL & 61.97 & 64.53 & \textbf{+0.194} \\
    Mistral-7B-Instruct-v0.3 & Qwen2.5-VL & 62.91 & 65.50 & +0.158 \\
    \midrule
    \textit{zero-shot} & GPT-5.4 & \textbf{73.94} & \textbf{75.28} & +0.216 \\
    Qwen3.5-9B & GPT-5.4 & 72.25 & 73.84 & +0.250$^{*}$ \\
    Qwen2.5-7B-Instruct & GPT-5.4 & 72.72 & 73.87 & +0.283$^{*}$ \\
    DeepSeek-R1-Distill-Llama-8B & GPT-5.4 & 72.47 & 73.76 & +0.270$^{*}$ \\
    Mistral-7B-Instruct-v0.3 & GPT-5.4 & 72.56 & 73.64 & \textbf{+0.293}$^{*}$ \\
    \bottomrule
  \end{tabular}
  \vspace{2pt}
  \begin{flushleft}
  \footnotesize{$^{*}$ marks $p<0.05$.}
  \end{flushleft}
\end{table}

% \begin{table}[t]
%   \centering
%   \caption{\small\textbf{Effect of structured physical prior source and evaluator.}
%   Each row is a pair of prior source and question evaluator.
%   \emph{zero-shot} means without the structured physical prior $K_s$.
%   \emph{Overall} and \emph{Weighted} are mean accuracies (\%) across four
%   T2V generators. $\Delta$ is relative to the zero-shot setting of the same
%   evaluator. $\rho_{\text{human}}$ is the scene-level Spearman correlation
%   with the human study.
%   Cross-source priors improve Qwen3.5-9B accuracy and improve GPT-5.4
%   human correlation, suggesting that the effect of $K_s$ is not merely due
%   to self-evaluation, but depends on evaluator capacity and prompt
%   compatibility.}
%   \label{tab:ablation_kb_eval}
%   \small
%   \setlength{\tabcolsep}{8pt}
%   \renewcommand{\arraystretch}{1.05}
%   \begin{tabular}{ll cccc}
%     \toprule
%     \textbf{$K_s$ source} & \textbf{Evaluator}
%     & \textbf{Overall} & \textbf{Weighted}
%     & \textbf{$\Delta$} & \textbf{$\rho_{\text{human}}$} \\
%     \midrule
%     \textit{zero-shot} & Qwen3.5-9B & 72.75 & 74.56 & +0.00 & +0.165 \\
%     Qwen3.5-9B & Qwen3.5-9B & \textbf{74.91} & \textbf{76.52} & \textbf{+2.16} & +0.201 \\
%     Qwen2.5-7B-Instruct & Qwen3.5-9B & 73.66 & 75.42 & +0.91 & +0.209 \\
%     DeepSeek-R1-Distill-Llama-8B & Qwen3.5-9B & 73.81 & 75.67 & +1.06 & \textbf{+0.251}$^{*}$ \\
%     Mistral-7B-Instruct-v0.3 & Qwen3.5-9B & 74.09 & 76.13 & +1.34 & +0.248$^{*}$ \\
%     \midrule
%     \textit{zero-shot} & Qwen2.5-VL & 63.47 & 65.89 & +0.00 & +0.015 \\
%     Qwen3.5-9B & Qwen2.5-VL & \textbf{66.09} & \textbf{69.00} & \textbf{+2.62} & +0.104 \\
%     Qwen2.5-7B-Instruct & Qwen2.5-VL & 63.25 & 66.15 & -0.22 & +0.156 \\
%     DeepSeek-R1-Distill-Llama-8B & Qwen2.5-VL & 61.97 & 64.53 & -1.50 & \textbf{+0.194} \\
%     Mistral-7B-Instruct-v0.3 & Qwen2.5-VL & 62.91 & 65.50 & -0.56 & +0.158 \\
%     \midrule
%     \textit{zero-shot} & GPT-5.4 & \textbf{73.94} & \textbf{75.28} & +0.00 & +0.216 \\
%     Qwen3.5-9B & GPT-5.4 & 72.25 & 73.84 & -1.69 & +0.250$^{*}$ \\
%     Qwen2.5-7B-Instruct & GPT-5.4 & 72.72 & 73.87 & -1.22 & +0.283$^{*}$ \\
%     DeepSeek-R1-Distill-Llama-8B & GPT-5.4 & 72.47 & 73.76 & -1.47 & +0.270$^{*}$ \\
%     Mistral-7B-Instruct-v0.3 & GPT-5.4 & 72.56 & 73.64 & -1.37 & \textbf{+0.293}$^{*}$ \\
%     \bottomrule
%   \end{tabular}
%   \vspace{2pt}
%   \begin{flushleft}
%   \footnotesize{$^{*}$ marks $p<0.05$.}
%   \end{flushleft}
% \end{table}

% \subsection{Correlation with Human Judgment}
% \label{subsec:comparisonHuman}

% \paragraph{Human validation.}
% Table~\ref{tab:human_validation} reports human validation on the 100-scene subset.
% The average human accuracy is 63.22\%, indicating that the questions are answerable but non-trivial for human observers.
% This is important because \phymetric{} is designed to test fine-grained physical consequences rather than obvious visual quality.
% The VLM evaluator achieves higher label accuracy under the full protocol, but we do not interpret this as video models or VLMs outperforming humans.
% Human annotators judge from visual evidence alone, while the automatic evaluator also receives a fixed question format and physics-grounded structured context.

% Human--VLM agreement averages 68.82\%.
% Scene-level Spearman correlations are positive for all four video models, with the strongest correlation on Cosmos-7B ($\rho=0.349$, $p=0.0004$) and a significant correlation on Wan2.2-14B ($\rho=0.223$, $p=0.0257$).
% The correlations are moderate rather than high, which reflects the difficulty of temporally grounded physical judgment.
% We therefore use the human study as validation of question clarity and evaluator alignment, not as a direct replacement for large-scale automatic evaluation.

% \begin{table}[t]
% \centering
% \caption{
% Human validation on the 100-scene subset.
% The subset contains two scenes from each of the 50 physical categories, yielding 800 binary questions.
% We report human accuracy against benchmark labels, VLM accuracy under the full protocol, human--VLM agreement, and scene-level Spearman correlation.
% }
% \label{tab:human_validation}
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{lccccc}
% \toprule
% Video model & Human Acc. & VLM Acc. & Agreement & Scene $\rho$ & $p$ \\
% \midrule
% CogVideoX-5B  & 61.38 & 70.62 & 68.75 & 0.136 & 0.1781 \\
% Cosmos-7B     & 60.38 & 76.50 & 66.38 & \textbf{0.349} & \textbf{0.0004} \\
% Wan2.1-1.3B   & 61.25 & 74.62 & 67.38 & 0.099 & 0.3290 \\
% Wan2.2-14B    & \textbf{69.88} & \textbf{77.88} & \textbf{72.75} & 0.223 & 0.0257 \\
% \midrule
% Average       & 63.22 & 74.91 & 68.82 & 0.202 & -- \\
% \bottomrule
% \end{tabular}
% \end{table}

% Table~\ref{tab:human_decomposition} further decomposes human--VLM outcomes.
% On average, humans and the VLM are jointly correct on 53.47\% of questions and jointly wrong on 15.35\%.
% The VLM-only region is larger than the human-only region, which is consistent with the higher VLM label accuracy in Table~\ref{tab:human_validation}.
% However, the human-only cases remain important: they indicate visible physical evidence that the VLM fails to use, and motivate future evaluator improvements.
% Wan2.2-14B has the highest joint-correct rate and the lowest joint-wrong rate, suggesting that better generated videos also lead to more stable agreement between human and automatic evaluation.


% \begin{table}[t]
% \centering
% \caption{
% Human--VLM outcome decomposition on the 100-scene subset.
% ``Human only'' denotes cases where humans match the benchmark label but the VLM does not.
% ``VLM only'' denotes cases where the VLM matches the label but humans do not.
% }
% \label{tab:human_decomposition}
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{lcccc}
% \toprule
% Video model & Both correct & Both wrong & Human only & VLM only \\
% \midrule
% CogVideoX-5B  & 50.38 & 18.38 & 11.00 & 20.25 \\
% Cosmos-7B     & 51.62 & 14.75 & 8.75  & 24.88 \\
% Wan2.1-1.3B   & 51.62 & 15.75 & 9.62  & 23.00 \\
% Wan2.2-14B    & \textbf{60.25} & \textbf{12.50} & 9.62 & 17.62 \\
% \midrule
% Average       & 53.47 & 15.35 & 9.75 & 21.44 \\
% \bottomrule
% \end{tabular}
% \end{table}




==> sections/06Discussion.tex <==
\section{Discussion}
\label{sec:discussion}


\subsection{Findings}
\label{subsec:findings}



\subsection{Limitations}
\label{subsec:limitaion}


